Image Reconstruction: From Sparsity to Data-adaptive Methods and Machine Learning

The field of medical image reconstruction has seen roughly four types of methods. The first type tended to be analytical methods, such as filtered back-projection (FBP) for X-ray computed tomography (CT) and the inverse Fourier transform for magnetic resonance imaging (MRI), based on simple mathematical models for the imaging systems. These methods are typically fast, but have suboptimal properties such as poor resolution-noise trade-off for CT. A second type is iterative reconstruction methods based on more complete models for the imaging system physics and, where appropriate, models for the sensor statistics. These iterative methods improved image quality by reducing noise and artifacts. The FDA-approved methods among these have been based on relatively simple regularization models. A third type of methods has been designed to accommodate modified data acquisition methods, such as reduced sampling in MRI and CT to reduce scan time or radiation dose. These methods typically involve mathematical image models involving assumptions such as sparsity or low-rank. A fourth type of methods replaces mathematically designed models of signals and systems with data-driven or adaptive models inspired by the field of machine learning. This paper focuses on the two most recent trends in medical image reconstruction: methods based on sparsity or low-rank models, and data-driven methods based on machine learning techniques.

==> bio-jcy.tex <==
 is currently a Professor of the Dept. of Bio/Brain Engineering and Adjunct Professor at Dept. of Mathematical Sciences of Korea Advanced Institute of Science and Technology (KAIST), Korea. He received the B.Sc. and M.Sc. degrees from Seoul National University, Korea, and the Ph.D. from Purdue University, West Lafayette.
From 1999 to 2001 he was a postdoc fellow at Coordindate Science Lab, University of Illinois at Urbrana-Champaign. From 2001 to 2004,  he worked at Philips Research and GE Global Research in New York. In 2004, he joined KAIST as an assistant professor, and he is now a Professor.  He has served as an associate editor of IEEE Trans. on Image Processing,  IEEE Trans. on Computational Imaging, Journal of Electronic Imaging,  an editorial board member for Magnetic Resonance in Medicine, and  an international advisory board member for Physics in Medicine and Biology. He is currently an associate editor for IEEE Trans. on Medical Imaging, a Senior Editor of IEEE Signal Processing Magazine, and a section editor of BMC Biomedical Engineering. He is  a vice-chair of IEEE SPS Technical Committee for Computational Imaging, and a general co-chair (with Mathews Jacob) for 2020 IEEE Symp. on Biomedical Imaging (ISBI), Iowa City. His group was the first place winner of the 2009 Recon Challenge at the ISMRM workshop, and the second place winner at 2016 Low Dose CT Grand Challenge organized by the American Association of Physicists in Medicine (AAPM). He was an advisor of best student paper awards (1st, and runner-up) at 2013 and 2016 IEEE Symp. on Biomedical Imaging (ISBI). His current research interests include machine learning and sparse recovery for various imaging reconstruction problems in x-ray CT, MRI, optics, ultrasound, etc.




==> bio-jf.tex <==
%Jeff Fessler
is the William L. Root Professor of EECS at the University of Michigan. He received the BSEE degree from Purdue University in 1985, the MSEE degree from Stanford University in 1986, and the M.S. degree in Statistics from Stanford University in 1989. From 1985 to 1988 he was a National Science Foundation Graduate Fellow at Stanford, where he earned a Ph.D. in electrical engineering in 1990. He has worked at the University of Michigan since then. From 1991 to 1992 he was a Department of Energy Alexander Hollaender Post-Doctoral Fellow in the Division of Nuclear Medicine. From 1993 to 1995 he was an Assistant Professor in Nuclear Medicine and the Bioengineering Program. He is now a Professor in the Departments of Electrical Engineering and Computer Science, Radiology, and Biomedical Engineering. He became a Fellow of the IEEE in 2006, for contributions to the theory and practice of image reconstruction. He received the Francois Erbsmann award for his IPMI93 presentation, and the Edward Hoffman Medical Imaging Scientist Award in 2013. He has served as an associate editor for the IEEE Transactions on Medical Imaging, the IEEE Signal Processing Letters, the IEEE Transactions on Image Processing, the IEEE Transactions on Computational Imaging, and is currently serving as an associate editor for SIAM J. on Imaging Science. He has chaired the IEEE T-MI Steering Committee and the ISBI Steering Committee. He was co-chair of the 1997 SPIE conference on Image Reconstruction and Restoration, technical program co-chair of the 2002 IEEE International Symposium on Biomedical Imaging (ISBI), and general chair of ISBI 2007. His research interests are in statistical aspects of imaging problems, and he has supervised doctoral research in PET, SPECT, X-ray CT, MRI, and optical imaging problems.

==> bio-sr.tex <==
received the B.Tech. degree in Electrical Engineering from the Indian Institute of Technology (IIT) Madras, India, in 2008, and the M.S. and Ph.D. degrees in Electrical and Computer Engineering in 2010 and 2014 respectively, from the University of Illinois at Urbana-Champaign. After his Ph.D., Dr. Ravishankar was an Adjunct Lecturer in the Department of Electrical and Computer Engineering, and a Postdoctoral Research Associate in the Coordinated Science Laboratory at the University of Illinois. From August 2015, he was a Research Fellow in the Department of Electrical Engineering and Computer Science at the University of Michigan, Ann Arbor. He was a Postdoc Research Associate in the Theoretical Division at Los Alamos National Laboratory from August 2018 to February 2019. He is currently an Assistant Professor in the Departments of Computational Mathematics, Science and Engineering, and Biomedical Engineering at Michigan State University. His research interests include signal and image processing, biomedical and computational imaging, data-driven methods, machine learning, signal modeling, inverse problems, data science, compressed sensing, and large-scale data processing. He was a recipient of the IEEE Signal Processing Society Young Author Best Paper Award for 2016. 
A paper he co-authored won a best student paper award at the IEEE International Symposium on Biomedical Imaging (ISBI), 2018, and another was a finalist at the IEEE International Workshop on Machine Learning for Signal Processing (MLSP), 2017.
He is currently a member of the IEEE Computational Imaging Technical Committee.



==> s,bio.tex <==
% s,bio

\newpage
%
\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.25in,clip,keepaspectratio]
{photo/SaiprasadRavishankar.pdf}}]
{Saiprasad Ravishankar}
\input{bio-sr.tex}
\end{IEEEbiography}
%\vspace{-2in}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]
{photo/jong.pdf}}]
{Jong Chul Ye}
\input{bio-jcy.tex}
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photo/fessler.pdf}}]{Jeffrey A. Fessler}
\input{bio-jf.tex}
\end{IEEEbiography}
